Provable Training for Graph Contrastive Learning

Graph Contrastive Learning (GCL) has emerged as a popular training approach for learning node embeddings from augmented graphs without labels. Despite the key principle that maximizing the similarity between positive node pairs while minimizing it between negative node pairs is well established, some fundamental problems are still unclear. Considering the complex graph structure, are some nodes consistently well-trained and following this principle even with different graph augmentations? Or are there some nodes more likely to be untrained across graph augmentations and violate the principle? How to distinguish these nodes and further guide the training of GCL? To answer these questions, we first present experimental evidence showing that the training of GCL is indeed imbalanced across all nodes. To address this problem, we propose the metric "node compactness", which is the lower bound of how a node follows the GCL principle related to the range of augmentations. We further derive the form of node compactness theoretically through bound propagation, which can be integrated into binary cross-entropy as a regularization. To this end, we propose the PrOvable Training (POT) for GCL, which regularizes the training of GCL to encode node embeddings that follows the GCL principle better. Through extensive experiments on various benchmarks, POT consistently improves the existing GCL approaches, serving as a friendly plugin.

==> src/graph-level.tex <==
\section{Extending POT to Graph-Level GCL}
We first define the common setting of graph-level GCL, which is designed for learning graph representations for graph-level downstream tasks. Suppose there are $N$ graphs in a batch when training, \{$G_1,G_2,\dots,G_N$\}. Two augmentations {$G_{n,i},G_{n_j}$} are sampled from the set of all possible augmentations $\mathcal G_n$, $n=1,2,\dots,N$. $h_{n,i}=f(X_n, A_{n,i})$ and $h_{n,j}=f(X_n, A_{n,j})$ are the graph embeddings, where $f:\mathcal X \times \mathcal A \rightarrow \mathbb R^d$ is the encoder. Graph-level GCL also follows InfoMax principle but in a different manner:
\begin{equation}
    l_n = -\log \frac{e^{\theta(h_{n,i},h_{n,j})/\tau}}{\sum_{n'\neq n}e^{\theta(h_{n',i},h_{n',j})/\tau}}
\end{equation}

To evaluate how a graph embedding follows InfoMax under possible augmentations, we extend the concept of node compactness in Definition~\ref{def: metric} to the following definition with repect to graph embeddings:

\begin{definition}[Graph Compactness]\label{def: gc}
    Let $f_\theta$ denote the encoder of graph-level GCL. The compactness of graph $n$ is defined as
    \begin{equation}
        \underline{\tilde f}_n = \min_{\substack{G_{n,i}=(X_n, A_{n,i})\\
            G_{n,j}=(X_n, A_{n,j})}}
             \{\frac{1}{N-1} \sum_{n' \neq n} h_{n,i} \cdot (\bar h_{n,j} - \bar h_{n',j})\ |\ h_{n,i}=f_\theta(X_n, A_{n,i}), h_{n,j}=f_\theta(X_n, A_{n,j})\}
    \end{equation}
    where $\bar h = h / \|h\|_2$ is the normalized vector.
\end{definition}
\begin{definition}[$i$-Graph Compactness]\label{def: gc-i}
    Under Definition~\ref{def: gc}, the compactness of graph $n$ in view $i$ is defined as
    \begin{equation}
        \underline{\tilde f}_{n,i} = \min_{G_{n,i}=(X_n, A_{n,i})} \{h_{n,i}W_n^{CL_G}\ |\ h_{n,i}=f_\theta(X_n, A_{n,i})\}
    \end{equation}
    where $W_n^{CL_G} = \bar h_{n,j} - \frac{1}{N-1} \sum_{n' \neq n}\bar h_{n',j}$ is constant.
\end{definition}
